Bayesian inference under differential privacy

Bayesian inference is an important technique throughout statistics. The essence of Beyesian inference is to derive the posterior belief updated from prior belief by the learned information, which is a set of differentially private answers under differential privacy. Although Bayesian inference can be used in a variety of applications, it becomes theoretically hard to solve when the number of differentially private answers is large. To facilitate Bayesian inference under differential privacy, this paper proposes a systematic mechanism. The key step of the mechanism is the implementation of Bayesian updating with the best linear unbiased estimator derived by Gauss-Markov theorem. In addition, we also apply the proposed inference mechanism into an online queryanswering system, the novelty of which is that the utility for users is guaranteed by Bayesian inference in the form of credible interval and confidence level. Theoretical and experimental analysis are shown to demonstrate the efficiency and effectiveness of both inference mechanism and online query-answering system.

==> data/Experiment_long.tex <==
\section{Experimental study}
\label{sec-exp}
\subsection{Experiment setup}
\textbf{Environment}
All experiments were run on a
computer with Intel P8600(2 * 2.4 GHz) CPU and 2GB memory.

\textbf{Data.} We use the three data sets: net-trace, social network and search logs, which are the same data sets with \cite{boost-accuracy}.
Net-trace is an IP-level network trace collected at
a major university; Social network is a graph of
friendship relations in an online social network site; Search
logs is a set of search query logs over time from Jan.1, 2004 to 2011.
The results of different data are similar, so we only show net-trace and search logs results for lack of space.

\textbf{Query.} User queries may not necessarily obey a certain distribution. So the question arises how to generate the testing queries.
In our setting, queries are assumed to be multinomial distributed,
which means the probability for the query to involve cell $x_j$ is $P_j$, where $\sum_{j=1}^n P_j=1$.
For efficiency and practicality, we assume there exist some regions of interest, where the cells are asked more frequently than others.
Equation (\ref{fml-Query-P}) shows the probability of each cell.
\begin{align}
\label{fml-Query-P}
P_j=0.9 * 10^{-floor(\frac{j-1}{10})}
\end{align}
where the function $floor()$ rounds the input to the nearest integers less than it.

To generate a query, we first generate a random number $n_t$ in $1\sim 10$, which is the $\#$ of independent trails of multinomial distribution.
Then we generate the query from the multinomial distribution, equation (\ref{fml-Q-Pr}) shows the probability of $Q$.
\begin{multline}
\label{fml-Q-Pr}
Pr(Q_1=q_1, Q_2=q_2,\cdots, Q_n=q_n)=\\\frac{n_t!}{q_1! q_2! \cdots q_n!} P_1^{q_1} P_2^{q_2}  \cdots P_n^{q_n}
\end{multline}
where $\sum_j q_j=n_t$.

Finally, we generate 1000 queries for each setting.


%longer_version_mark
\textbf{Utility Requirement}
We assume each query has different utility requirement ($\epsilon$,$\delta$).
%We need to select the utility requirement $\epsilon$ and $\delta$ in definition \ref{definition-usefulness} carefully to run the experiment due to the computation complexity.
Intuitively, the larger $\epsilon$ (or the smaller $\delta$) , the smaller $\alpha$ allocated because of theorem \ref{theo-budget-allocation}, then the wider probability function of noise.
To simulate the estimation process with high accuracy, $m_d$ in theorem \ref{theo-complexity-2} becomes larger.
Then the computation complexity may becomes too high. Therefore, we assume the upper bound of $\epsilon$ is $10^4$.
In the following sub-sections, $\epsilon$ is uniformly distributed.


\textbf{Settings and Metrics.}
The main innovations of this paper include the method of dynamic privacy budget allocation, Bayesian inference and how to implement them to a real system.
Therefore,
we conduct three settings of experiments to demonstrate these three methods.

Besides system privacy cost $\bar{\alpha}$
in theorem \ref{theo-privacy-cost}, following metrics are used.

For a bounded system, Once the system privacy cost $\bar{\alpha}$ reaches the overall privacy budget, then the system cannot answer further queries.
To measure this feature, we define the ratio of answered queries as below. In another word, it indicates the capacity(or life span) of a system.
\begin{definition}
\label{def-answer-ratio}
Under the bound of overall privacy budget, given a set of query \textbf{Q} with utility requirements, the answer ratio $R_a$ is
\begin{align}
R_a=\frac{(\#\ of\ answers:\ Pr(L\leq \theta \leq U)\geq 1-\delta)}{(\#\ of\ all\ queries)}
\end{align}
\end{definition}


\begin{figure}[htbp]
\centering
\includegraphics[height=3cm]{privacy_cost_for_dynamic_allocation_unif1000_nettrace.pdf}
\includegraphics[height=3cm]{privacy_cost_for_dynamic_allocation_unif1000_search.pdf}
%\caption{}
%\label{fig-allocation-privacy-nettrace}
\includegraphics[height=3cm]{utility_ratio_for_dynamic_allocation_unif1000_nettrace.pdf}
\includegraphics[height=3cm]{utility_ratio_for_dynamic_allocation_unif1000_search.pdf}
\caption{Evaluation of dynamic budget allocation for net-trace(left) and search logs(right). All x-axes represent $\#$ of queries. First row
shows $\bar{\alpha}$; second row shows $R_i$.}
\label{fig-dynamic-budget-alloc}
\end{figure}

%To show the impact of dynamic $\alpha$ allocation,
%we define the metric ratio of satisfaction $R_s$ measure the utility of data,
Among all the {\bf answered queries}, we want to know the accuracy of the returned answer.
We use following two metrics.
1. $R_i$ is defined to show whether the returned interval really contain the original answer;
2. $E$ is the defined to indicate the distance between returned answer and true answer.
It's easy to prove that if $\#$ of answered queries approaches to infinity, $R_i$ converges to confidence level.

\begin{definition}
\label{def-ratio-of-satisfaction}
For a set of queries with utility requirements, the credible intervals $[L,U]$ are returned.
Ratio of reliability $R_i$ is defined as follows:
\begin{align}
R_i=\frac{\#\ of\ answers:\ L\leq \theta \leq U}{\#\ of\ all\ answered\ queries}
\end{align}
\end{definition}


\begin{definition}
\label{def-relative-error}
For each query with ($\epsilon,\delta$) requirement, a returned answer $\hat{\theta}$ is provided by the query answering system.
If the original answer is $\theta$,
the relative error is defined to reflect the accuracy of $\hat{\theta}$:
\begin{align}
\label{eqn-relative-error}
E=\frac{\sum_{i \in answered\ queries}(|\hat{\theta}_i-\theta_i|/\epsilon_i)}{\#\ of\ all\ answered\ queries}
\end{align}
\end{definition}

In summary, $\bar{\alpha}$ indicates the system privacy cost; $R_a$ indicates the capacity(or life span) of a system;
$R_i$ indicates the confidence level of returned credible interval $[L,U]$; $E$ indicates the accuracy of the point estimation $\hat{\theta}$.









\subsection{Evaluation of dynamic budget allocation}
To evaluate the method of dynamic budget allocation, we compare it with the traditional static budget allocation method.
Let $\epsilon$ be uniformly distributed in $[50,10^4]$, overall privacy budget be 4, $\delta=0.05$.

By dynamic budget allocation, we only spend necessary budget corresponding each query's utility requirement. Therefore,
in Figure \ref{fig-dynamic-budget-alloc}, the $R_i$ of dynamic allocation achieves best utility, but less budget $\bar{\alpha}$ has been spent.
Because $\bar{\alpha}$ hasn't reached the bound 4, $R_a=1$(budget is not exhausted).







\subsection{Evaluation of Bayesian inference}
To facilitate the method of Bayesian inference, first, a hierarchical partitioning tree\cite{boost-accuracy} is given using 0.3-differential privacy
as query history to help infer queries; second, the overall privacy budget is set as 6.
Let $\epsilon$ be uniformly distributed in $[50,10^3]$, $\delta=0.2$.

We improve the baseline interactive query-answering system with dynamic budget allocation, then it can save privacy budget and achieve better utility.
Then the improved baseline systems are compared with or without Bayesian inference technique.
Because we don't allocate privacy budget if the estimate can satisfy utility requirement, privacy budget can be saved furthermore.
In Figure \ref{fig-impact-inference}, $R_i$ and $E$ also become better using inference technique.
Because overall budget is 6, so $R_a=1$.

%We can see that dynamic budget allocation exhaust fewer budget than static budget allocation.

%
%Next we show the utility result about inference in Figure \ref{fig-unbounded-utility}. As number of queries increases, more and more observations
%can be derived to make inference of a target query, the error declines gradually as the ``inference'' line.


\begin{figure}
\centering
\includegraphics[height=3cm]{System_privacy_for_unbounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{System_privacy_for_unbounded_system4_search.pdf}
%\label{fig-system-privacy-unbounded-nettrace}
\includegraphics[height=3cm]{Avg_abs_error_for_unbounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{Avg_abs_error_for_unbounded_system4_search.pdf}
%\label{fig-system-privacy-unbounded-search}
\includegraphics[height=3cm]{R_range_for_unbounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{R_range_for_unbounded_system4_search.pdf}
%\label{fig-system-privacy-unbounded-social}
\caption{Evaluation of Beyesian inference for net-trace(left) and search logs(right). All x-axes represent $\#$ of queries.
First row shows $\bar{\alpha}$; second row shows $E$; third row shows $R_i$. Improved baseline means baseline system with dynamic budget allocation.}
\label{fig-impact-inference}
\end{figure}
\begin{figure}
\centering
\includegraphics[height=3cm]{Answer_ratio_for_bounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{Answer_ratio_for_bounded_system4_search.pdf}
%\label{fig-answer-ratio-bounded-nettrace}
\includegraphics[height=3cm]{Avg_abs_error_for_bounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{Avg_abs_error_for_bounded_system4_search.pdf}
%\label{fig-answer-ratio-bounded-search}
\includegraphics[height=3cm]{R_range_for_bounded_system4_nettrace.pdf}
\includegraphics[height=3cm]{R_range_for_bounded_system4_search.pdf}
%\label{fig-answer-ratio-bounded-social}
\caption{Evaluation of real bounded system for net-trace(left) and search logs(right). All x-axes represent $\#$ of queries.
First row shows $R_a$; second row shows $E$; third row shows $R_i$. Improved baseline and
LS solution are improved by our method of dynamic budget allocation.
}
\label{fig-real_sys}
\end{figure}
\begin{figure}
\centering
\includegraphics[height=3cm]{Impact_alpha_to_ratio_epsilon1000_nettrace.pdf}
\includegraphics[height=3cm]{Impact_alpha_to_ratio_epsilon1000_search.pdf}
%\label{fig-impact-alpha-nettrace}
\includegraphics[height=3cm]{Impact_alpha_to_error_epsilon1000_nettrace.pdf}
\includegraphics[height=3cm]{Impact_alpha_to_error_epsilon1000_search.pdf}
%\label{fig-impact-alpha-search}
\includegraphics[height=3cm]{Impact_alpha_to_range_epsilon1000_nettrace.pdf}
\includegraphics[height=3cm]{Impact_alpha_to_range_epsilon1000_search.pdf}
%\label{fig-impact-alpha-social}
\caption{Impact of overall privacy budget for net-trace(left) and search logs(right). All x-axes represent overall privacy budget.
First row shows $R_a$; second row shows $E$; third row shows $R_i$.
$\epsilon$ is uniformly distributed in $[1,10^3]$.}
\label{fig-impact-privacy-budget}
\end{figure}


\subsection{Evaluation of online bounded system}
\label{cha:exp-evaluation-real-system}
For a bounded system, we use dynamic budget allocation and Bayesian inference to improve the performance.
We set the overall privacy budget as $1$.
Let $\epsilon$ be uniformly distributed in $[1,10^3]$, $\delta=0.2$. Figure \ref{fig-real_sys} shows the performance.
%
%Because the bound of $\bar{\alpha}$, only limited queries can be answered by the online system. If adopting our statistical inference,
%queries can also be inferred by the query history; otherwise for ordinary system, only the same query in query history can be answered after the system privacy reaches the bound.
%

Because $\bar{\alpha}$ reaches the overall privacy budget, $\bar{\alpha}=1$. Further queries cannot be answered by improved baseline system. But for our inference system,
it may also be answered by making inference of query history. This can increase $R_a$. Also $E$ and $R_i$ is better than improved baseline system.
We also compared $E$ of LS solution\cite{Optimizing-PODS} using dynamic budget allocation method.
In our setting, the result is better than LS solution because LS is not sensitive to
utility requirement and privacy cost $\alpha$. For example, if a query requires high utility, say $\epsilon=5$, then a big $\alpha$ is
allocated and a small noise is added to the answer. But LS solution treats all noisy answers as points without any probability feature.
Therefore, this answer with small noise contributes not so much to the LS estimate. Then according to Equation \ref{eqn-relative-error},
$E$ becomes lager than the inference result.

Note that $E$ and $R_i$ is not as good as Figure \ref{fig-impact-inference}. There are two reasons. First, we don't have any
query history at the beginning. So the system must build a query history to make inference for new queries. Second,
when $\bar{\alpha}$ reaches the overall privacy budget, the query history we have is actually the previous answered queries,
which are generated randomly. Compared with the hierarchical partitioning tree\cite{boost-accuracy}, it may not work so well.
We believe delicately designed query history\cite{SDMpaper,Optimizing-PODS,boost-accuracy} or auxiliary queries\cite{iReduct}
can improve our system even better, which can be investigated in further works.



\subsubsection{Impact of parameters}
We study the impact of overall privacy budget and utility requirement for the randomly generated 1000 queries.
Let $\delta=0.2$.
Figure \ref{fig-impact-privacy-budget} and \ref{fig-impact-query-distribution} show the results.
As overall privacy budget increases, or utility requirement declines, $R_a$ rises.
%Note that when overall budget is small
However, $E$ and $R_i$ are not effected
because they are derived from the answered queries. Although less queries are answered, the utility is still guaranteed.
%
%Note that when overall budget is small, or $\epsilon$ distribution is bounded in a small range, the results are not stable because
%$\bar{\alpha}$ reaches the bound of overall budget very soon.
%\textbf{Impact of overall privacy budget}

\begin{figure}
\centering
\includegraphics[height=3cm]{Impact_epsilon_to_ratio_alpha1_nettrace.pdf}
\includegraphics[height=3cm]{Impact_epsilon_to_ratio_alpha1_search.pdf}
%\label{fig-impact-epsilon-nettrace}
\includegraphics[height=3cm]{Impact_epsilon_to_error_alpha1_nettrace.pdf}
\includegraphics[height=3cm]{Impact_epsilon_to_error_alpha1_search.pdf}
%\label{fig-impact-epsilon-search}
\includegraphics[height=3cm]{Impact_epsilon_to_range_alpha1_nettrace.pdf}
\includegraphics[height=3cm]{Impact_epsilon_to_range_alpha1_search.pdf}
%\label{fig-impact-epsilon-social}
\caption{Impact of utility requirement for net-trace(left) and
search logs(right). All x-axes represent the upper bound of
$\epsilon$. For example, 200 means $\epsilon$ is uniformly
distributed in $[1,200]$. First row shows $R_a$; second row shows
$E$; third row shows $R_i$. overall privacy budget is 1.}
\label{fig-impact-query-distribution}
\end{figure}
















\subsection{Experiment conclusion}
The proposed system with dynamic privacy budget allocation and Bayesian inference outperforms baseline system(even with dynamic budget allocation).
Privacy cost $\bar{\alpha}$ increases slower for two reasons. First, once a query can be estimated from
query history, $\bar{\alpha}$ won't increase at all; Second, we only allocate the necessary budget for the query, which saves
privacy budget. $R_a$, $E$ and $R_i$ show that the utility is also better than improved baseline and LS solution because we assume
each query has different utility requirement, while LS solution is insensitive with privacy cost and utility requirement.
When overall privacy budget increases, or utility requirement declines, $R_a$ rises.
Delicately designed query history\cite{SDMpaper,Optimizing-PODS,boost-accuracy} or auxiliary queries\cite{iReduct}
can improve our system even better.


==> data/Figure.tex <==
\begin{align*}
Q_1=
\left[
\begin{array}{ccccccccc}
1&0&0&0&0&0&0&0&0
\end{array}
\right]
\\
Q_1 \textbf{x}=x_1
\\
\mathcal{A}_{Q_1}=Q_1\textbf{x}+\tilde{N}(\alpha/S_{Q_1})
\\
S_{Q_1}=1
\\
\tilde{N}(\alpha/S_{Q_1})=\tilde{N}(\alpha/1)
\\
\mathcal{A}_{Q_1}=10+\tilde{N}(\alpha)
\end{align*}


==> data/Related.tex <==
\section{Related works}

Online query answering system with differential privacy has been proposed for a long time\cite{Dwork-calibrating,Dwork-dp,McSherry-PINQ}.
However, researches about how to deal with the privacy budget was not conducted so much.
\cite{XX-outputperturbation} gives a useful techniques, called query relaxation, which returns an alternative answer of the original answer when
the original query is similar to some queries in history.

Many works on differential privacy and linear counting queries have been
proposed so far. \cite{Optimizing-PODS,Adaptive-query-strategy} provides a matrix mechanism
to release data when the workload of queries is already known.
\cite{boost-accuracy} hierarchically partitions one-dimensional data
and release the count of each cell. By checking the noisy counts
with the requirement of consistency, it boosts the accuracy of
release counts. \cite{SDMpaper} uses a KD-tree to partition and release the histograms.
\cite{Improving-utility-PCA} propose a PCA method to improve the utility, and \cite{DBLP:conf/icde/XiaoWG10}
uses wavelet to release data. All the above studies focus on absolute error. \cite{iReduct} propose an
algorithm to reduce relative error. Although these works can achieve optimal point estimation, interval estimation
has not been used.

 In the field of statistics, differential
privacy and statistics have been
researched\cite{Adam-MLE-estimator,McSherry-Probabilistic-inference,Dwork-robust-statistics,dwork2010differential-statistics}.
It's shown that accuracy of query answers can be boosted by
statistical inference, like maximal likelihood
estimator(MLE)\cite{Adam-MLE-estimator}, or the probabilistic
inference\cite{McSherry-Probabilistic-inference}.
\cite{Dwork-robust-statistics} talks about robust statistics.

Differential privacy makes assumptions that attackers know all but
one records in the data
set\cite{Kifer-no-free-lunch,diff-privacy-Bayesian,diff-privacy-statistical-database}.
It's proven in \cite{diff-privacy-Bayesian}that differential privacy
satisfies Bayesian probability.
\cite{diff-privacy-statistical-database} proved that differential
privacy limits the maximum information gain of an attacker from a
Bayesian perspective as controlling the ratio of posterior to prior
distributions. Similarly, \cite{Rastogi-adversarial-privacy} proved
that to some extent differential privacy is equivalent to
adversarial privacy, which is also a function of attacker's
posterior distribution. However, how to quantify the posterior
distribution has not been studied so far. Also, How much information
an attacker can gain from a differentially private answer is not
known in the literature. The Bayesian inference method of this paper
is an independent tool, which  can also be used for other tasks,
like disclosure risk analysis, parameter estimation and other
statistical inferences.
%
%We assume nobody knows the true answer except the data manager. Therefore, neither for users nor for adversaries, they cannot predict
%$Pr(\hat{\theta}|\theta)$. Otherwise, \cite{McSherry-Probabilistic-inference} gives the bounds of this equation derived from Jensen's Inequality.


==> data/chap03_long.tex <==
\section{Greedy online algorithm}
\label{sec-online}

\begin{figure}
\hspace{-1cm}
\includegraphics[width=11cm]{Query_answer_flow.pdf}
\vspace{-3.3cm}
\caption{Query answering flowchart}
\label{fig-query-flowchart}
\end{figure}

%Suppose currently we have a query history as Equation (\ref{fml-H}).
This section explains the query-answering mechanism. As shown in Figure \ref{fig-query-flowchart}, for any query $Q$, we need a utility
requirement in $(\epsilon,\delta)$.
At the beginning, we know the query history $\textbf{H}$, perturbed answers $\textbf{y}$ providing $\textbf{A}$-differential privacy\footnote{Which means each $y_i$ is $A_i$-differentially private.} and a
target query $Q$.
First,
(1) we find the observations(linear representations), denoted as $\tilde{\Theta}$(section \ref{cha3:sec-LP});
(2) posterior probability function and point estimation $\hat{\theta}$  can be
derived from $\tilde{\Theta}$ to satisfy Minimal Mean Square Error(section \ref{cha3:sec-query-estimation});
(3) next we can compute the credible interval(section \ref{cha3:sec-error});
if the utility is better than required, then output the estimate;
(4) else we generate the necessary privacy cost(section \ref{cha3:sec-budget-allocation}).
(5) then we evaluate the system privacy cost(section \ref{cha3:sec-privacy-cost});
(6) if answering this query will not overspend the overall privacy budget, then
invoke the query mechanism to return a differentially private answer $\tilde{\theta}$; else the system cannot provide an answer for $Q$ to satisfy the required utility.

In summary, the input is query $Q$ and utility requirement ($\epsilon,\delta$). The output can be one of the following:
the inference mechanism gives a point estimate $\hat{\theta}$ with minimal mean square error and an interval estimate $(L, U)$;
the query mechanism gives a query answer $\tilde{\theta}$ and an interval $(\tilde{\theta}-\epsilon, \tilde{\theta}+\epsilon)$.

This query answering flow is summarized in Algorithm \ref{alg-frame}.

%We postpone the technical details of probability function computation in section \ref{cha3:sec-query-estimation} to section \ref{sec-simulation-PDF}.



%\begin{equation}
%\small
%\small
%\label{fml-Q}
%\begin{array}{c}
%Q
%\end{array}
%\left[
%\begin{tabular}{c
%ccc
%>{\columncolor{yellow}}c
%>{\columncolor{yellow}}c
%ccc}
%0 &0& 0& 0& 1& 1& 0& 0& 0
%\end{tabular}
%\right]
%\sim
%\left[
%\begin{tabular}{l}
%0.06
%%$\frac{-ln \delta}{\epsilon}$
%\end{tabular}
%\right]
%\end{equation}


\begin{algorithm}
\caption{Online query-answering framework}
\begin{algorithmic}
\label{alg-frame}
%\textbf{Ëã·¨ \ref{alg-MMSE}£º}¼ÆËãת»»¾ØÕó$\textbf{B}$\\\hline
\REQUIRE{$Q$, $\epsilon, \delta$}\\
\IF{$\exists$ linear representation of $Q$}
\STATE (1) Find observations $\tilde{\Theta}$ by Algorithm \ref{alg-ob-MMSE};\\
(2) Estimate $\hat{\theta}$ by Algorithm \ref{alg-MMSE};\\
(3) Compute the credible interval by Algorithm \ref{alg-usefulness};
\ENDIF
\IF{utility is better than required}
\STATE return $\hat{\theta}$ and $(L,U)$;\\
\ELSE
\STATE Predict necessary privacy cost $\alpha$ by Theorem \ref{theo-budget-allocation};\\
\IF{answering this query won't overspend budget}
\STATE
$L\leftarrow\tilde{\theta}-\epsilon$; $U\leftarrow\tilde{\theta}+\epsilon$;\\
Return direct query answer $\tilde{\theta}$ and $(L,U)$;\\
Update $\textbf{H},\textbf{A},\textbf{B},\textbf{y}$;\\
\ELSE
\STATE No answer can be returned;
\ENDIF

\ENDIF
\RETURN{$\hat{\theta},L(\tilde{\Theta}),U(\tilde{\Theta})$}
\end{algorithmic}
\end{algorithm}





\subsection{Data model and example}
\label{cha3:sec-model-intro}

In this online model, the data manager needs to maintain the following information: query history matrix ${\bf H}$,
returned answers $\textbf{y}$ of ${\bf H}$ and used privacy cost $\textbf{A}$ for $\textbf{y}$.
%local privacy cost of each cell, denoted by $\textbf{B}$
%and the system privacy cost denoted by $\bar{\alpha}$.

\subsubsection{Data}%
%We use a ``data cube'' to represent the data space $\mathcal{D}^n$. We denote any sub-cube that is not divided by any more dimensions by
%``cell'', meaning it's the ``smallest'' sub-cube.
%For any multi-dimensional data cube, we can map data into one-dimensional vector, denoted by $\textbf{x}$.
%For example, we use the original data shown in {\bf Figure \ref{Fig_exampledata}} with attributes age and income.
%The domain value of age is $20\scriptsize{\sim}30$, $30\scriptsize{\sim}40$ and $40\scriptsize{\sim}50$; the domain value of income is $0\scriptsize{\sim}10K$, $10K\scriptsize{\sim}20K$ and $>20K$.
%We can represent the data in a multi-dimensional OLAP (Online Analytical Processing) data cube.  {\bf Figure \ref{Fig_exampledata}} shows the data represented in a two-dimensional count cube or histogram, in which each cell represents the population count corresponding to the age and income values.
%%A {\em generalized cube} can be constructed by grouping (generalizing) multiple cells into mutually disjoint partitions (sub-cubes).
%We can also represent the cells in the original data cube by a vector $\textbf{x}$ as equation (\ref{eqn_x}).

Consider a dataset with $N$ nominal or discretized attributes, we use an $N$-dimensional data cube,
also called a base cuboid in the data warehousing literature \cite{JWH-dataming,Ding:2011:DPD:1989323.1989347},
to represent the aggregate information of the data set.  The records are the points in the $N$-dimensional data space.
Each cell of a data cube represents an aggregated measure, in our case, the count of the data points corresponding to
the multidimensional coordinates of the cell. We denote the number of cells by $m$ and
$m = |dom(A_1)| * \dots * |dom(A_N)|$ where $|dom(A_i)|$ is the domain size of attribute $A_i$.
We use the term ``partition'' to refer to any sub-cube in the data cube.


\vspace{-0.5cm}
\begin{figure}[h!]
\centering
\hspace{-0.8cm}
\includegraphics[width=10cm]{Fig_exampledata.pdf}
\vspace{-4cm}
\caption{\small Example original data represented in a relational table (left) and a 2-dimensional count cube (right)}
\label{Fig_exampledata}
\end{figure}



{\bf Figure \ref{Fig_exampledata}} shows an example relational dataset with attribute age and income (left) and a two-dimensional
count data cube or histogram (right). The domain values of age are $20\scriptsize{\sim}30$, $30\scriptsize{\sim}40$ and $40\scriptsize{\sim}50$;
the domain values of income are $0\scriptsize{\sim}10K$, $10K\scriptsize{\sim}20K$ and $>20K$.
Each cell in the data cube represents the population count corresponding to the age and income values.
We can represent the original data cube, e.g. the counts of all cells, by an $m$-dimensional column vector $\textbf{x}$ shown below.
\begin{small}
\begin{equation}
\label{eqn_x}
\textbf{x}=
\left[
\begin{array}{ccccccccc}
10&21&37&20&50&40&53&0&0
\end{array}
\right]^T
\end{equation}
\end{small}

\vspace{-0.5cm}
\subsubsection{Query}
We consider linear counting queries that compute a linear combination of the count values in the data cube based on a query predicate.

\begin{definition}[Linear query \cite{Optimizing-PODS}] A linear query Q can be represented as an $m$-dimensional boolean vector $\textbf{Q} = [q_1 \dots q_n]$ with each $q_i \in \mathbb{R}$.  The answer to a linear query $\textbf{Q}$ on data vector $\textbf{x}$ is the vector product $\textbf{Qx}$ = $q_1x_1 + \dots + q_nx_n$.
\end{definition}

For example, If we know people with $income<10K$ don't pay tax, people with $10K<income<20K$ pay 1K dollars, people with $income>20K$ pay 2K dollars,
and from the total tax revenue 50K dollars are invested for education each year,  then
to calculate the total tax, following query Q2 can be issued.
\begin{itemize}
\item
Q2:    select 1K$*$count() where $10K<income<20K$ \\
    + 2K$*$count() where $income>20K$\\
    $-$ 50K
\end{itemize}
\begin{align}
\label{fml-query-Q2}
\begin{small}
Q2=\left[
\begin{array}{ccccccccc}
2 &2&2&1&1&1&0&0&0
\end{array}
\right]
\end{small}
\end{align}
\vspace{-0.5cm}
\begin{align}
\label{fml-AQ2}
\mathcal{A}_{Q2}=Q2 \cdot \textbf{x}+\tilde{N}(\alpha/S_{Q2})
\end{align}
Q2 has sensitivity 2 because any change of 1 record can affect the result by 2 at most.
Note that the constant 50K does not affect the sensitivity of Q2 because it won't vary for any record change
\footnote{$\mathcal{A}_{Q2}-50K$ would be the same with $\mathcal{A}_{Q2}'=Q2 \cdot\textbf{x}-50K+\tilde{N}(\alpha/S_{Q2})$, so we ignore the constant in $Q2$.}.
This feature is important for privacy budget composition discussed in section \ref{cha3:sec-privacy-cost}.
Equation (\ref{fml-query-Q2}) shows the query vector of Q2.
The returned answer $\mathcal{A}_{Q2}$
 from Laplace mechanism are shown in equation (\ref{fml-AQ2}) where $\alpha$ is the privacy cost of $Q2$.



\begin{definition} [Query matrix \cite{Optimizing-PODS}] A query matrix is a collection of linear queries, arranged by rows to form a
$p \times m$ matrix.
\end{definition}
Given a $p \times m$ query matrix \textbf{H}, the query answer for \textbf{H} is a length-$p$ column vector of query results, which can be computed as the matrix product \textbf{Hx}.
For example, an $m \times m$ identity query matrix $\textbf{I}_m$ will result in a length-$m$ column vector consisting of all the cell counts in the original data vector \textbf{x}.

%Below is important; it's the source for the figure \ref{Fig_model_illu}
%\vspace{-0.5cm}
%\begin{align}
%Q2=
%\left[
%\begin{array}{ccccccccc}
%2 &2&2&1&1&1&0&0&0
%\end{array}
%\right]
%\\
%Q2\cdot\textbf{x}=2x_1+2x_2+2x_3+x_4+x_5+x_6=226
%\\
%\tilde{\theta}_{Q_2}=Q2\cdot\textbf{x}+\tilde{N}(\alpha/S_{Q_2})
%\\
%S_{Q_2}=2
%\\
%\tilde{N}(\alpha/S_{Q_2})=\tilde{N}(\alpha/2)
%\\
%\tilde{\theta}_{Q_2}=226+\tilde{N}(\alpha/2)
%\end{align}



\vspace{-.3cm}
\begin{figure}[h!]
\centering
%\hspace{-.8cm}
\includegraphics[width=9cm]{Fig_model_illustration.pdf}
\vspace{-3.6cm}
\caption{Example of $\textbf{H}$ and $\textbf{y}$}
\label{Fig_model_illu}
\end{figure}


\subsubsection{Query history and Laplace mechanism}
%
%If a query can be estimated using statistical inference from the previous query answers with the satisfied utility, we don't invoke the differentially private query mechanism.
%Only when the query cannot be estimated, or the utility of estimate does not meet the utility requirement, we use the Laplace mechanism to obtain
%a differentially private answer. Then the answer will be added to query history\footnote{Note that query history only contains the queries whose answers are derived from Laplace mechanism.} to estimate future queries.
For different queries, sensitivity of each query vector may not be necessarily the same.
Therefore, we need to compute the sensitivity of
each query  by Lemma \ref{lemma-GS}.

\begin{lemma}
\label{lemma-GS}
For a linear counting query $Q$, the sensitivity of $Q$ is $max(abs(Q))$.
\end{lemma}
We use the function ``$abs()$'' to denote the absolute value of a vector, meaning that for all $j$, $[abs(Q)]_j=|Q_j|$.
$max(abs(Q))$ means the maximal value of $abs(Q)$.


If many queries have been issued already, then we can write the above equations in matrix form.
Let $\textbf{y}$, $\textbf{H}$, $\textbf{A}$ and $\textbf{S}$ be the matrix form of
$\mathcal{A}_Q$, $Q$, $\alpha$ and $S$ respectively. According to Lemma \ref{lemma-GS}, $\textbf{S}=max_{row}(abs(\textbf{H}))$
where $max_{row}(abs(\textbf{H}))$ is a column vector whose item is the maximal value of each row in $abs(\textbf{H})$.

Equations(\ref{fml-y}, \ref{fml-SH}) summarize the relationship of $\textbf{y}$, $\textbf{H}$, $\textbf{x}$, $\tilde{\textbf{N}}$ and $\textbf{A}$.
\begin{align}
\label{fml-y}
\textbf{y}=\textbf{Hx}+\tilde{\textbf{N}}(\textbf{A}./\textbf{S})
\\
\label{fml-SH}
\textbf{S}=max_{row}(\textbf{abs(\textbf{H})})
\end{align}
where
operator ./ means $\forall i$,
$[\textbf{A}./\textbf{S}]_i=A_i/S_i$.


\subsubsection{Running example}
Suppose we have a query history matrix $\textbf{H}$ as equation (\ref{fml-H}), $\textbf{x}$ as equation (\ref{eqn_x})
and the privacy parameter $\textbf{A}$ used in all query vector shown in equation (\ref{fml-A}).



\begin{align}
\small
\label{fml-H}
\textbf{H}=
\left[
\begin{tabular}{c
ccc
c
c
ccc}
0 & 1 &0 &0 &1 &0&0&0&0\\
0 & 0 &0 &0 &0 &0&0&1&1\\
0 & 0 &0 &0 &4 &2&0&0&0\\
0 & 0 &0 &0 &2 &0&0&0&0\\
0 & 0 &0 &0 &1 &1&0&-1&-1\\
0 & 1 &0 &0 &0 &0&0&0&0\\
0 & 0 &0 &0 &0 &2&0&0&0\\
\end{tabular}
\right]
\end{align}
\begin{align}
\label{fml-A}
\textbf{A}=
\left[
\begin{tabular}{ccccccc}
0.05&
    0.1&
    0.05&
    0.1&
    0.1&
    0.05&
    0.05
\end{tabular}
\right]^T
\end{align}

Then according to Lemma \ref{lemma-GS}, $\textbf{S}$ can be derived in equation (\ref{fml-S}).
\begin{align}
\label{fml-S}
\textbf{S}=\left[
\begin{array}{ccccccc}
1& 1& 4& 2& 1& 1& 2
\end{array}
\right]^T
\end{align}

Therefore, the relationship of $\textbf{y}$, $\textbf{H}$, $\textbf{A}$ and $\textbf{S}$ in equation (\ref{fml-y}) can be illustrated in equation (\ref{fml-HI-color})
%\begin{align}
%\label{fml-yHAS}
%%\begin{tabular}{cp{25pt}cp{110pt}cp{80pt}}
%%\centering $\textbf{y}$=&\textbf{Hx}+&$\tilde{N}$($\textbf{A}./\textbf{S}$)
%%\end{tabular}
%\textbf{y}=\textbf{Hx}+\tilde{N}(\textbf{A}./\textbf{S})
%\end{align}
%\vspace{-.5cm}
\begin{align}
\tiny
\label{fml-HI-color}
%\textbf{(HI)}=
\left[
\begin{array}{c}
y_1\\
y_2\\
y_3\\
y_4\\
y_5\\
y_6\\
y_7\\
\end{array}
\right]
=
\left[
\begin{tabular}{c
ccc
c
c
ccc}
0 & 1 &0 &0 &1 &0&0&0&0\\
0 & 0 &0 &0 &0 &0&0&1&1\\
0 & 0 &0 &0 &4 &2&0&0&0\\
0 & 0 &0 &0 &2 &0&0&0&0\\
0 & 0 &0 &0 &1 &1&0&-1&-1\\
0 & 1 &0 &0 &0 &0&0&0&0\\
0 & 0 &0 &0 &0 &2&0&0&0\\
\end{tabular}
\right]
\textbf{x}
+
\tilde{\tiny{N}}
\left(
\begin{tabular}{l}
0.05/1\\
    0.1/1\\
    0.05/4\\
    0.1/2\\
    0.1/1\\
    0.05/1\\
    0.05/2\\
\end{tabular}
\right)
\end{align}

With above $\textbf{y}$, $\textbf{H}$, $\textbf{A}$ and $\textbf{S}$,
assume the target query $Q\textbf{x}$ is $x_5+x_6$ with utility requirement as $(\epsilon=15,\delta=0.2)$.
Then
\begin{align}
\label{fml-Q}
Q=\left[
\begin{array}{ccccccccc}
0&0&0&0&1&1&0&0&0
\end{array}
\right]
\end{align}





























\subsection{Bayesian inference}
Equation (\ref{fml-HI-color}) is essentially a system of linear equations which could be overdetermined and inconsistent.
Linear least squares (LS) approach approximately solves the  overdetermined system with a solution $\hat{\textbf{x}}$.
Given a query $\textbf{Q}$, the answer to $\textbf{Q}$ is $\textbf{Q}\hat{\textbf{x}}$ and does not provide a query specific utility guarantee.

Our Bayesian inference approach, on the other hand, attempts to find answer to $\textbf{Q}\textbf{x}$ by solving the equation $\textbf{TH}=\textbf{Q}$.
For each solution $T_i$, $T_i\textbf{H}$ provides a linear representation of $\textbf{Q}$, which has the form in Equation (\ref{fml-Tilde-theta}).
Note $N_i$ can be composed Laplace noise, which may NOT be Laplace noise.
Given the solution of $\textbf{T}$ and the set of observations, we can find an optimal estimate and credible interval
for $\textbf{Qx}$(also called $\theta$ in this paper).
\begin{align}
\label{fml-Tilde-theta}
\tilde{\theta}_i=Q\textbf{x}+N_i
\\
\label{fml-tilde-textbf-N}
N_i=T_i\tilde{\textbf{N}}_i
\end{align}

Section \ref{cha3:sec-LP} describes how we find $\textbf{T}$;
Section \ref{cha3:sec-query-estimation} describes how we compute the estimate $\hat{\theta}$ for Qx based on the set of observations;
Section \ref{cha3:sec-error} describes how to find the credible interval.

\subsubsection{Linear representation of a query}
\label{cha3:sec-LP}
%We denote the matrix of query history by ${\bf H}$, the user query by $Q$,
%
%Equations (\ref{fml-Tilde-theta}) and (\ref{fml-tilde-textbf-N}) are our goal.


If multiple observations can be found, it's an overdetermined linear problem.
However, finding all the possible linear representations is NP-hard. Even if we assume the
rows of $\textbf{H}$ are linearly independent, there are $\frac{m!}{(n!)^{m/n}}$ possible sets of solutions where
$\textbf{H}\in \mathbb{R}^{m\times n}$.

Theorem \ref{theo-ob-NP} proves the computational complexity.
If finding the optimal estimate for one query is NP-hard, then finding optimal estimates for a bunch of queries are also NP-hard.
\begin{theorem}
\label{theo-ob-NP}
Finding all the possible linear representations of query $Q$ from query history $\textbf{H}$ is NP-hard.
\end{theorem}
\begin{proof}
This problem can be transformed to $k$-partition problem\cite{k-partition-NP}.
Without loss of generality, we assume $\textbf{H}\in \mathbb{R}^{nk\times n}$ and all rows of $\textbf{H}$ are linear independent.

Let $\textbf{H}$ be a set and each row be an element. First we can randomly partition $\textbf{H}$ into
$n$ sets of $k$ cardinalities. If we can partition $\textbf{H}$ into $k$ sets of cardinality $n$, then each set is
a solution of $\textbf{Q}$ because they are linear independent.
Because $k$-partition problem is NP-hard, this problem is NP-hard.
\end{proof}

For computation simplicity, we use a greedy approach to derive the linear representations.
We start from the first row of H, repeatedly search through the first $k$ rows of H, denoted by $\textbf{H}(1 : k)$,
until we find a solution $T_i$ for $T_i \textbf{H}(1:k) = \textbf{Q}$.
Then add
$T_i\textbf{H}$ to the observation $\tilde{\Theta}$.
Next we replace the involved rows of $\textbf{H}$ with row vector $\textbf{0}$.
In another word, if $T_{ij} \neq 0$, then $\textbf{H}_j$ is involved, replace $\textbf{H}_j$ with $\textbf{0}$.
 Next we find $T_{i+1}$ similarly.
Algorithm \ref{alg-ob-MMSE} summarizes the process.



%In our example, equation (\ref{fml-HI-color}) is the result of step 2. The yellow columns
%are the target columns; the gray rows are the target rows.
%Equation (\ref{fml-ob-color}) and (\ref{fml-ob-example}) are the results of step 3 and 4. According to step 5, we combine $x_2$ and $x_6$ to one row and allocate $\alpha_3=0.05$ to them.
%In step 6, we need to calculate budget cost of each observation. For example, $\tilde{\theta}_1$ doesn't involve any new query, so $BC(\tilde{\theta}_1)=0$;
%$\tilde{\theta}_3$ involves two cells with $0.05$, so $BC(\tilde{\theta}_3)=0.1$. Finally, we output $\tilde{\theta}_1$ because
%$\tilde{\theta}_1$ and $\tilde{\theta}_2$ have least $BC$ and $\tilde{\theta}_1$ has bigger $\alpha_i$ than $\tilde{\theta}_2$.
%Note that in each iteration, we need to update the maintaining information $\textbf{H},\textbf{y},\textbf{A}$ and $\textbf{B}$.


\begin{algorithm}
\caption{Search observations $\tilde{\Theta}$} %with $\textbf{T}$, $\textbf{A}$, $\textbf{y}$}
\begin{algorithmic}
\label{alg-ob-MMSE}
%\textbf{Ëã·¨ \ref{alg-MMSE}£º}¼ÆËãת»»¾ØÕó$\textbf{B}$\\\hline
\REQUIRE{$Q$, $\textbf{H}$, $\textbf{y}$, $\textbf{A}$}\\
%$\textbf{H}_{copy}, \textbf{A}_{copy}, \textbf{y}_{copy}\leftarrow \textbf{H}, \textbf{A}, \textbf{y}$;
$[m, n]=size(\textbf{H})$;\\
$i \leftarrow 1$;\\
\FOR{($k=1$; $k \leq m$; $k=k+1$)}
\IF{$T*\textbf{H}(1:k)=Q$ has solution for T}
\STATE
$\textbf{T}_i=Q/\textbf{H}(1:k)$;\\
Add $\textbf{T}_i$ to $\textbf{T}$ as a row;\\
%Remove involved rows from $\textbf{H}$: \\
\{ for all $j$,
\IF{$T_{ij} \neq 0$}
    \STATE Replace $\textbf{H}_j$ with row vector $\textbf{0}$;\\
\ENDIF \\
\}\\
$i\leftarrow i+1$;\\
\ENDIF \\
\ENDFOR
\RETURN{$\tilde{\Theta}$, $\textbf{T}$}
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{theo-Ty-Theta}
Let $\tilde{\Theta}$ be the observations of target query $Q$, then
\begin{align}
\tilde{\Theta}=\textbf{Q x}+\textbf{T}\tilde{\textbf{N}}\\
\textbf{N}=\textbf{T}\tilde{\textbf{N}}
\end{align}
\end{theorem}

\begin{proof}
\begin{align}
\textbf{Ty}=\textbf{T}(\textbf{Hx}+\tilde{\textbf{N}})
=\textbf{THx}+\textbf{T}\tilde{\textbf{N}}
=\textbf{Qx}+\textbf{T}\tilde{\textbf{N}}
\end{align}
It's the sum of original answer $\textbf{Qx}$ and a composed noise. So $\tilde{\Theta}=\textbf{Qx}+\textbf{T}\tilde{\textbf{N}}$, $\textbf{N}=\textbf{T}\tilde{\textbf{N}}$.
\end{proof}



Let's consider the running example $Q$ in equation (\ref{fml-Q}).
First $i=1$. When $i$ increases to $4$, $T*\textbf{H}(1:4)=Q$ has solution for $T_1$, $T_1=[0\ 0\ (1/2)\ (-1/2)\ 0\ 0\ 0]$. Denote the first observation as $\tilde{\theta}_1$, $\tilde{\theta}_1=T_1\textbf{y}$ is in equation (\ref{fml-T1-H}).
The involved rows of $\textbf{H}$ is shown in the yellow rows in equation (\ref{fml-HI-color2}).

\begin{multline}
\label{fml-T1-H}
\small
\tilde{\theta}_1=T_1\textbf{y}=y_3/2-y_4/2\\
=
{(H_3\textbf{x}+\tilde{N}(A_3/S_3))/2-(H_4\textbf{x}+\tilde{N}(A_4/S_4))/2}\\
=Q\textbf{x}+\frac{\tilde{N}(A_3/S_3)-\tilde{N}(A_4/S_4)}{2}
\end{multline}
\begin{align}
\label{fml-HI-color2}
\small
%\textbf{(HI)}=
\left[
\begin{array}{c}
y_1\\
y_2\\
\rowcolor{yellow}y_3\\
\rowcolor{yellow}y_4\\
y_5\\
y_6\\
y_7\\
\end{array}
\right]
=
\left[
\begin{tabular}{c
ccc
c
c
ccc}
0 & 1 &0 &0 &1 &0&0&0&0\\
0 & 0 &0 &0 &0 &0&0&1&1\\
\rowcolor{yellow}0 & 0 &0 &0 &4 &2&0&0&0\\
\rowcolor{yellow}0 & 0 &0 &0 &2 &0&0&0&0\\
0 & 0 &0 &0 &1 &1&0&-1&-1\\
0 & 1 &0 &0 &0 &0&0&0&0\\
0 & 0 &0 &0 &0 &2&0&0&0\\
\end{tabular}
\right]
\textbf{x}
+
\tilde{\textbf{N}}
%\left[
%\begin{tabular}{l}
%0.05/1\\
%    0.1/1\\
%\rowcolor{yellow}    0.05/4\\
% \rowcolor{yellow}   0.1/2\\
%    0.1/1\\
%    0.05/1\\
%    0.05/2\\
%\end{tabular}
%\right]
\end{align}

Because we know the value of $\textbf{y}$, $\textbf{A}$ and $\textbf{S}$, then it can be written in
\begin{align}
\tilde{\theta}_1=Q\textbf{x}+N_1=(y_3-y_4)/2=-16.7\\
N_1=\frac{\tilde{N}(0.05/4)-\tilde{N}(0.1/2)}{2}
\end{align}
Above equations show that the target query $Q$ can be linearly represented by the query history $\textbf{H}$ with the feature that noise would be {\bf composed of many Laplace noises}.

 Next we replace these rows with vector $\textbf{0}$
and find $T_2$ similarly in Equation (\ref{fml-HI-color3}). When $i$ increases to 5, $T\textbf{H}(1:5)=Q$ has a solution for $T_2$, which is $[0\ 1\ 0\ 0\ 1\ 0\ 0]$.

To find all the linear representations(observations), we have
\begin{align}
\tilde{\theta}_2=y_2+y_5=Q\textbf{x}+N_2=1.1\\
N_2=\tilde{N}(0.1/1)-\tilde{N}(0.1/1)\\
\tilde{\theta}_3=y_1-y_6+y_7/2=Q\textbf{x}+N_3=-11.5\\
N_3=\tilde{N}(0.05/1)-\tilde{N}(0.05/1)+\frac{\tilde{N}(0.05/2)}{2}
\end{align}





%Because the first two elements of $\textbf{T}_1$ are 0, we remove the first two rows in $\textbf{T}_1$,
%$\textbf{A}_{L1}$ and $\textbf{y}_{L1}$. Then $\textbf{H}_{copy}$ and $\textbf{A}_{copy}$ are shown in equation (\ref{fml-H-copy}).
%$\tilde{\theta}_1$ is shown in equation (\ref{fml-ob-example-1}), (\ref{fml-ob-example-2}) and (\ref{fml-ob-example-3}).
\begin{align}
\small
\label{fml-HI-color3}
%\textbf{(HI)}=
\left[
\begin{array}{c}
y_1\\
\rowcolor{yellow}y_2\\
y_3\\
y_4\\
\rowcolor{yellow}y_5\\
y_6\\
y_7\\
\end{array}
\right]
=
\left[
\begin{tabular}{c
ccc
c
c
ccc}
0 & 1 &0 &0 &1 &0&0&0&0\\
\rowcolor{yellow}0 & 0 &0 &0 &0 &0&0&1&1\\
0 & 0 &0 &0 &0 &0&0&0&0\\
0 & 0 &0 &0 &0 &0&0&0&0\\
\rowcolor{yellow}0 & 0 &0 &0 &1 &1&0&-1&-1\\
0 & 1 &0 &0 &0 &0&0&0&0\\
0 & 0 &0 &0 &0 &2&0&0&0\\
\end{tabular}
\right]
\textbf{x}
+
\tilde{\textbf{N}}
%\left[
%\begin{tabular}{l}
%0.05/1\\
%\rowcolor{yellow}    0.1/1\\
%    0.05/4\\
%    0.1/2\\
%\rowcolor{yellow}    0.1/1\\
%    0.05/1\\
%    0.05/2\\
%\end{tabular}
%\right]
\end{align}
Finally, $\textbf{T}$, $\tilde{\Theta}$ are shown in the yellow part of equation (\ref{fml-T}) and equation \ref{fml-Ty-example}.
\begin{align}
\label{fml-T}
\textbf{TH}=
\left[
\begin{array}{ccccccc}
\rowcolor{yellow}0&0&1/2&-1/2&0&0&0\\
\rowcolor{yellow}0&1&0&0&1&0&0\\
\rowcolor{yellow}1&0&0&0&0&-1&1/2
\end{array}
\right]
\textbf{H}
=\left[
\begin{array}{c}
Q\\
Q\\
Q
\end{array}
\right]
\\
\label{fml-Ty-example}
\begin{tiny}
\tilde{\Theta}
=\theta+
\small
\left[
\begin{array}{c}
({\tilde{N}(0.05/4)-\tilde{N}(0.1/2)})/2\\
\small
\tilde{N}(0.1/1)-\tilde{N}(0.1/1)\\
\tiny
\tilde{N}(0.05/1)-\tilde{N}(0.05/1)+\frac{\tilde{N}(0.05/2)}{2}
\end{array}
\right]
=
\left[
\begin{array}{c}
-16.7\\
1.1\\
-11.5
\end{array}
\right]
\end{tiny}
\end{align}

%
%
%
%\begin{align}
%\label{fml-ob-example-1}
%\textbf{A}_{L1}=[0.05\ 0.1]^T;\ \textbf{T}_1=[1\ 1];\ \textbf{y}_{L1}=[y_3\ y_4];\\
%\label{fml-ob-example-2}
%\tilde{\theta}_1=\textbf{T}_1*\textbf{y}_{L1}=y_3+y_4=Q\textbf{x}+\textbf{T}_1*\tilde{\textbf{N}}(\textbf{A}_{L1})\\
%\label{fml-ob-example-3}
%\textbf{T}_1*\tilde{\textbf{N}}(\textbf{A}_{L1})=\tilde{N}(0.05)+\tilde{N}(0.1);
%\end{align}
%
%Similarly, we can find $\tilde{\theta}_2$ and $\tilde{\theta}_3$ as equation (\ref{fml-ob-example}) and (\ref{fml-ob-example-5}).
%\begin{small}
%\begin{align}
%\label{fml-ob-example}
%\tilde{\theta}_2=-y_2+y_5=Q\textbf{x}+\tilde{N}(0.1)-\tilde{N}(0.1)\\
%\label{fml-ob-example-5}
%\tilde{\theta}_3=y_1-y_6+y_7=Q\textbf{x}+\tilde{N}(0.05)-\tilde{N}(0.05)+\tilde{N}(0.05)
%\end{align}
%\end{small}
%
%Equation (\ref{fml-ob-color}) summarizes the three observations of $Q$.
%\begin{equation}
%\small
%\small
%\hspace{-5pt}
%\label{fml-ob-color}
%\begin{array}{r}
%y_3\\
%y_4\\
%\hline
%-y_2\\
%+y_5\\
%\hline
%y_1\\
%-y_6\\
%+y_7\\
%\end{array}
%\left[
%\begin{tabular}{c
%ccc
%>{\columncolor{yellow}}c
%>{\columncolor{yellow}}c
%ccc}
%0 & 0 &0 &0 &0 &1&0&0&0\\
%0 & 0 &0 &0 &1 &0&0&0&0\\
%\hline
%0 & 0 &0 &0 &0 &0&0&1&1\\
%0 & 0 &0 &0 &1 &1&0&1&1\\
%\hline
%0 & 1 &0 &0 &1 &0&0&0&0\\
%0 & 1 &0 &0 &0 &0&0&0&0\\
%0 & 0 &0 &0 &0 &1&0&0&0\\
%\end{tabular}
%\right]
%\sim
%\left[
%\begin{tabular}{l}
%    0.05\\
%    0.1\\
%    \hline
%0.1\\   0.1\\
%\hline
%       0.05\\
%    0.05\\
%0.05\\
%\end{tabular}
%\right]
%\end{equation}
%\begin{tabular}{p{175pt}p{40pt}}
%\centering\textbf{(H)}&($\textbf{A}$)
%\end{tabular}


































\subsubsection{Bayesian inference}
\label{cha3:sec-query-estimation}
We have all observations of the query in this step. To estimate the answer,
we formulate the problem as a Bayesian estimation problem
to seek $argmin_{\hat{\theta}}$($\mathbb{E}[(\hat{\theta}-\theta)^2]$) where operator $argmin_{\hat{\theta}}$
means to find the argument $\hat{\theta}$ to achieve the minimal value of $\mathbb{E}[(\hat{\theta}-\theta)^2]$, $\theta$ is the true value of
query and $\hat{\theta}$ is the estimate of the query. %Note that observations with different $\alpha$ can also be solved by our method.
%Our task is to find $argmin_{\hat{\theta}}(\mathbb{E}[\hat{\theta}-\theta)^2|\tilde{\Theta}]$.
According to the MMSE estimator\cite{book-statistical-inference}, our goal is to obtain
\begin{align}
\label{fml-hat-theta}
\hat{\theta}=\mathbb{E}(\theta|\tilde{\Theta})=\mathbb{E}(\theta|\tilde{\theta}_1,\tilde{\theta}_2,\cdots,\tilde{\theta}_n).
\end{align}

So the next question is how to compute the expectation value given the observed answers?
There are several ways to solve the problem. Because we need not only the estimate but also the credible interval,
we should calculate the probability function of the estimate $\hat{\theta}$.


In the rest of this section, we need to process many probability functions. So we denote $f_Z(z)$ a probability function of $Z$, $f_Z(x)$ a probability function of $Z$ with input variable $x$.
For example, if $f_{\tilde{N}}(x)$ is the probability function of $\tilde{N}(\alpha)$ whose probability function is shown in equation (\ref{fml-Laplace-distribution}),
$f_{\tilde{N}}(z)$ is shown in the following equation.
\begin{align}
\label{fml-Laplace-distribution-z}
f_{\tilde{N}}(z)=\frac{\alpha}{2}exp(-{\alpha |z|});
\end{align}%

Theorem \ref{theo-PDF-iteration} gives a way to compute the probability function
iteratively.
\begin{theorem}
\label{theo-PDF-iteration}
Let $f_i(\theta)=Pr(\theta|\tilde{\theta}_1,\tilde{\theta}_2,\cdots,\tilde{\theta}_i)$,
%$\\=Pr(\theta|\tilde{\Theta}_i)$.
\begin{align}
\label{fml-PDF-theta-iteration}
f_i(\theta)=f_{i-1}(\theta)\frac{Pr(\tilde{\theta}_i|\theta)}{Pr(\tilde{\theta}_i)}
\end{align}
\end{theorem}
%
%\begin{proof}
%\begin{align*}
%Pr(\theta|\tilde{\Theta}_{l-1},\tilde{\theta}_l)=\frac{Pr(\theta)Pr(\tilde{\Theta}_{l-1}|\theta)Pr(\tilde{\Theta}_l|\theta)}{Pr(\tilde{\Theta}_{l-1})Pr(\tilde{\theta}_l)}\\
%=\frac{Pr(\tilde{\Theta}_{l-1})Pr(\theta|\tilde{\Theta}_{l-1})Pr(\tilde{\theta}_l|\theta)}{Pr(\tilde{\Theta}_{l-1})Pr(\tilde{\theta}_l)}\\
%=\frac{Pr(\theta|\tilde{\Theta}_{l-1})Pr(\tilde{\theta}_l|\theta)}{Pr(\tilde{\theta}_l)}\\
%=Pr_{l-1}(\theta)\frac{Pr(\tilde{\theta}_l|\theta)}{Pr(\tilde{\theta}_l)}
%\end{align*}
%\end{proof}
Therefore, we can calculate $f_n(\theta)$ from $\tilde{\theta}_1$ to $\tilde{\theta}_n$ iteratively. Note that when $i=1$, we assume $f_0(\theta)$ is uniformly distributed\cite{book-statistical-inference},
meaning that $f_1(\theta)=f(\tilde{\theta}_1|\theta)$. So the next question is how to derive $Pr(\tilde{\theta}_i|\theta)$.
Theorem \ref{theo-theta-N} shows a way to solve this.

\begin{theorem}
\label{theo-theta-N}
Let $f_{N_i}()$ be the probability function of $N_i$ in Equation (\ref{fml-Tilde-theta}),
meaning $N_i$ is the composed noise of each observation, then
\begin{align}
\label{fml-theta-N}
Pr(\tilde{\theta}_i|\theta)=f_{N_i}(\tilde{\theta}_i-\theta)
\end{align}
\end{theorem}
\begin{proof}
\begin{align}
Pr(\tilde{\theta}_i|\theta)=f(\tilde{\theta}_i=\theta+N_i|\theta)=f(N_i=\tilde{\theta}_i-\theta|\theta)
\end{align}
Note that the shape of $f_{N_i}()$ doesn't change with $\theta$, therefore,
\begin{align}
f(N_i=\tilde{\theta}_i-\theta|\theta)=f_{N_i}(\tilde{\theta}_i-\theta)
\end{align}
\end{proof}

\begin{theorem}
Equations (\ref{fml-corallary-PDF-theta}, \ref{fml-corollary-hat-theta}) are the Bayesian estimator achieving MMSE.
\begin{align}
\label{fml-corallary-PDF-theta}
f_\theta(\theta|\tilde{\Theta})=\prod_{i}\frac{f_{N_i}(\tilde{\theta}_i-\theta)}{f(\tilde{\theta}_i)}
\end{align}
\begin{align}
\label{fml-corollary-hat-theta}
\hat{\theta}=\int \theta \prod_{i}\frac{f_{N_i}(\tilde{\theta}_i-\theta)}{f(\tilde{\theta}_i)}d\theta
\end{align}
where $f(\tilde{\theta}_i)=\int f(\tilde{\theta}_i | \theta)d\theta$.
\end{theorem}

Given the above theorems, we will be capable to derive the Bayesian estimate to achieve MMSE as long as we know the probability function of $f_{N_i}()$
in equation (\ref{fml-Tilde-theta}). However, $N_i$ is a composed noise which may not be Laplace distributed. For example, in equation
(\ref{fml-Ty-example}), $N_1=({\tilde{N}(0.05/4)-\tilde{N}(0.1/2)})/2$ is a linear result of Laplace noises.




Next we show the theoretical probability function of linear composition of Laplace noises in Equation (\ref{fml-baliteral-gamma}).
\begin{theorem}[\cite{Bilateral-gamma}]
The probability function of sum of n i.i.d Laplace noises is
\begin{small}
\begin{align}
\label{fml-baliteral-gamma}
f_n(z)=\frac{\alpha^{n}}{2^n  \Gamma^2(n)}exp(-{\alpha |z|})\int_0^{\infty}v^{n-1}(|z|+\frac{v}{2\alpha})^{n-1}e^{-v}dv
\end{align}
\end{small}
\end{theorem}

Note that above equation is just the case when each $\alpha$ is the same. More complicated equations with different $\alpha$
can be found in \cite{book-Laplace}.

Because it's too difficult to calculate the theoretical probability function, we use a simulation approach to derive it.
Detailed and sophisticated techniques about simulation approach can be found in \cite{book-statistical-inference,book-probability-models,book-Laplace}.
%longer_version_mark
Our simulation algorithm is described in Section \ref{sec-simulation-PDF}.
Here we assume we have the result of $f_{N_i}()$.

Then by Theorem \ref{theo-theta-N}, $f(\tilde{\theta}_i|\theta)$ can be derived; by Theorem \ref{theo-PDF-iteration}, $f_i(\theta)$ can be derived iteratively;
by Equation (\ref{fml-corollary-hat-theta}) the $\hat{\theta}$ can be derived.
Algorithm \ref{alg-MMSE} summarizes the estimation process.
%$Pr_i(\theta)=Pr(\theta|\tilde{\theta}_1,\tilde{\theta}_2,\cdots,\tilde{\theta}_i)$.
%At the beginning, we use uniform distribution as $Pr_0(\theta)$.
%Because of the complexity of PDF computation, we leave the detailed techniques to section \ref{sec-simulation-PDF}.

\begin{algorithm}
\caption{Bayes estimation to achieve MMSE}
\begin{algorithmic}
\label{alg-MMSE}
\REQUIRE{$\tilde{\Theta}$, $\textbf{T}$, $\textbf{y}$}\\
%$i \leftarrow 1$;\\
$[m,n]=size(\tilde{\Theta})$;
\FOR{($i=1;i<n;i=i+1$)}
%longer_version_mark
\STATE Compute $f_{N_i}()$ by Algorithm \ref{alg-simulation-PDF} or Algorithm \ref{alg-combination-PDF};\\
        Compute $Pr(\tilde{\theta}_i|\theta)$ by Theorem \ref{theo-theta-N};
\ENDFOR
\STATE Derive $\hat{\theta}$ by equation (\ref{fml-corollary-hat-theta}), $f_\theta(\theta | \tilde{\Theta})$ by equation (\ref{fml-corallary-PDF-theta});
\\
\RETURN{$\hat{\theta}$, $f_\theta(\theta| \tilde{\Theta})$}
\end{algorithmic}
\end{algorithm}

In our example, $\textbf{T}$ and $\tilde{\Theta}$ are shown in equations (\ref{fml-T}, \ref{fml-Ty-example}). There are 3 observations.
So $f(\tilde{\theta}_1|\theta)$, $f(\tilde{\theta}_2|\theta)$ and $f(\tilde{\theta}_3|\theta)$ can be calculated.
The probability function curves are shown in Figure \ref{fig-query-answering-example}.
And the probability function of $f_\theta(\theta| \tilde{\Theta})$ is shown in the solid line. By equation (\ref{fml-hat-theta}),
we know that  $\theta$ lies in $[68,102]$ with probability $80\%$, $\hat{\theta}=84$.

%Note that the estimated PDF may not necessarily be symmetric, which means MLE\cite{Adam-MLE-estimator} may be different from MMSE estimator although
%both are unbiased.

\begin{figure}
\hspace{-.3cm}
\includegraphics[width=9cm]{MMSE_example_for_paper_new.pdf}
\vspace{-.8cm}
\caption{Query answering example, $\tilde{\theta}_1=73.34;\ \tilde{\theta}_2=91.12;\ \tilde{\theta}_3=78.46;\ \hat{\theta}=84;$ with $80\%$ probability in $[68,102]$.}
\label{fig-query-answering-example}
\end{figure}






























































\subsubsection{Credible interval}
\label{cha3:sec-error}
In this step, we have the posterior probability function, the question is
how to compute the credible interval.

For credible interval, we formulate the problem as following:
given the confidence level $1-\delta$, how to find the narrowest interval containing probability $1-\delta$?
Many classical solutions can be found in \cite{book-statistical-inference,book-probability-models,book-Laplace}.
To reduce the computational complexity, we assume the credible interval will contain the point estimation $\hat{\theta}$.
Then by integrating
the probability mass(density) to $1-\delta$, we can find the credible interval. Algorithm \ref{alg-usefulness} summarizes the process, which uses probability function in discrete domain.

\begin{algorithm}
\caption{credible interval}
\begin{algorithmic}
\label{alg-usefulness}
\REQUIRE{$\hat{\theta}$, probability function: $Pr_\theta(\theta|\tilde{\Theta})$, $\delta$}\\
\STATE 1. $a\leftarrow \hat{\theta}$; $b \leftarrow 0$; $P_m\leftarrow 0$;\\
2. \WHILE{$P_m<1-\delta$}
\IF{$Pr_\theta(a)\geq Pr_\theta(a+b)$}
\STATE $P_m\leftarrow P_m+Pr_\theta(a)$; $a\leftarrow a-1$; $b \leftarrow b+1$;\\
\ELSE
\STATE $P_m\leftarrow P_m+Pr_\theta(a+b)$; $b \leftarrow b+1$;\\
\ENDIF
\ENDWHILE
\\
\STATE 3. $L(\tilde{\Theta})\leftarrow a;$ $U(\tilde{\Theta}) \leftarrow b$.
\RETURN{$L(\tilde{\Theta})$, $U(\tilde{\Theta})$}
\end{algorithmic}
\end{algorithm}


%From these observations, we estimate $\hat{\theta}=1.72$ with probability $80\%$ in $[-22, 12]$.
 In our example, recall that the required range size is 15*2=30 with probability $80\%$.
 However, the credible interval size is $102-68=34$.
 Thus the error is bigger than required.
 Unfortunately we need to invoke the differentially private query mechanism, which is discussed in section \ref{cha3:sec-dp-mechanism}.

%
%Following theorems show the error of the MMSE point estimation.
%Theorem \ref{theo-error-epsilon} shows the unbiasedness.
%Theorem \ref{theo-absolute-error} and \ref{theo-MSE} give the absolute error and mean square error.
%\begin{theorem}
%\label{theo-error-epsilon}
%MMSE estimator is unbiased.
%\end{theorem}
%\begin{proof}
%$\operatorname{E}[\hat{\theta}]=\operatorname{E}[\operatorname{E}[\theta|\tilde{\Theta}]]=\theta$
%\end{proof}
%
%
%\begin{lemma}
%\label{lamma-PDF-epsilon}
%Denote $|\hat{\theta}-\theta|$ as $\gamma$, then
%\begin{align}
%\label{fml-PDF-epsilon}
%\operatorname{Pr}_\gamma(\gamma)=2\operatorname{Pr}_\theta(\hat{\theta}+\gamma)=2\operatorname{Pr}_\theta(\hat{\theta}-\gamma)
%\end{align}
%\end{lemma}
%\begin{proof}
%$\operatorname{Pr}_\gamma(\gamma)=\operatorname{Pr}_\gamma(|\hat{\theta}-\theta|)=\operatorname{Pr}_\theta(\hat{\theta}-\theta)+\operatorname{Pr}_\theta(\hat{\theta}+\theta)=2\operatorname{Pr}_\theta(\hat{\theta}+\gamma)=2\operatorname{Pr}_\theta(\hat{\theta}-\gamma)$
%\end{proof}
%
%
%
%
%\begin{theorem}
%\label{theo-absolute-error}
%The absolute error of our estimator is
%\begin{align}
%\label{fml-absolute-error}
%\operatorname{E}[\gamma]=2\int_{-\infty}^{\hat{\theta}}(\hat{\theta}-\theta)Pr_\theta(\theta)d\theta=2\int_{\hat{\theta}}^{\infty}(\theta-\hat{\theta})Pr_\theta(\theta)d\theta
%\end{align}
%\end{theorem}
%\begin{proof}
%Using equation (\ref{fml-PDF-epsilon}) can get the direct result.
%\end{proof}
%
%
%\begin{theorem}
%\label{theo-MSE}
%MSE of our estimator is
%\begin{align}
%\label{fml-MSE}
%\operatorname{MSE}(\hat{\theta})=%2\int_0^\infty \epsilon^2 Pr_\theta(\hat{\theta}+\epsilon)d\epsilon=
%2\int_0^\infty \gamma^2 \prod_{i}\frac{Pr_{\tilde{N}_i}(\tilde{\theta}_i-\hat{\theta}-\gamma)}{Pr(\tilde{\theta}_i)}d\gamma
%\end{align}
%\end{theorem}
%\begin{proof}
%\begin{align}
%\label{fml-error-MSE}
%\operatorname{MSE}(\hat{\theta})=\operatorname{E}[\gamma^2]=\int_0^\infty \gamma^2 Pr_{\gamma}(\gamma)d\gamma
%\end{align}
%From equations (\ref{fml-PDF-epsilon}) and (\ref{fml-corallary-PDF-theta}), we can derive equation (\ref{fml-MSE}).
%\end{proof}
%
%





































\subsection{Differentially private query mechanism}
\label{cha3:sec-dp-mechanism}
Only when the utility of estimate does not meet the requirement, we need to invoke the differentially private query mechanism,
return $\mathcal{A}(D)$ and interval $[\mathcal{A}(D)-\epsilon, \mathcal{A}(D)+\epsilon]$ to user,
add the query $Q$ to query history $\textbf{H}$, noisy answer $\mathcal{A}(D)$ to $\textbf{y}$ and allocated budget $\alpha$ to $\textbf{A}$.


\subsubsection{Budgeted query answering}
\label{cha3:sec-budget-allocation}
The first step is to decide how much necessary privacy cost should be allocated. Theorem \ref{theo-budget-allocation} shows the solution which spends
$S_Q \frac{-ln\delta}{\epsilon}$ privacy cost.
\begin{theorem}
\label{theo-budget-allocation}
Given the utility requirement $\epsilon, \delta$ of a query $Q$, it's enough to allocate $\alpha=S_Q \frac{-ln\delta}{\epsilon}$.
\end{theorem}
\begin{proof}
Let $\mathcal{A}_Q(D)=Q(D)+\tilde{N}(\alpha/S_Q)$.
Because probability function of laplace distribution is symmetric, in definition \ref{definition-usefulness}, $[\mathcal{A}(D)-\epsilon, \mathcal{A}(D)+\epsilon]$ gives the most probability mass.
\begin{multline}
\label{fml-budget-allocation-1}
Pr(-\epsilon\leq \mathcal{A}_Q(D)-Q(D)\leq \epsilon)\\
=Pr(-\epsilon\leq \tilde{N} \leq \epsilon)\\
=\int_{-\epsilon}^{\epsilon}\frac{\alpha/S_Q}{2}exp(-{\alpha/S_Q |x|})dx\\
=2\int_{-\epsilon}^0 \frac{\alpha/S_Q}{2}exp({\alpha/S_Q x})dx\\
=1-exp(-\frac{\epsilon \alpha/S_Q}{2})\geq 1-\delta \quad
\end{multline}
So we have $\alpha\geq S_Q \frac{-ln\delta}{\epsilon}$.
\end{proof}

In our example, we obtain that $\alpha=0.108$ would be enough, then we assume $A_8=0.108$ and $H_8=Q$.







\subsubsection{Privacy cost evaluation}
\label{cha3:sec-privacy-cost}

Next we solve the privacy budget cost of the system to test whether the privacy cost is within overall privacy budget in a bounded differentially private system if answering the query $Q$.
If no, no answer can be returned to user for security reason; otherwise, we return the differentially private answer from Laplace mechanism using the
derived necessary privacy cost and update the system parameters $\textbf{H}$, $\textbf{A}$ and $\textbf{y}$ for the next coming query.


In this paper, we assume the cells of the data are independent or only have negative correlations
\cite{Rastogi-adversarial-privacy}.
Generally speaking, this means adversaries cannot infer the count answer of a cell from any other cells. specifically, cells are independent if they
do not have any correlation at all; cells are negative correlated\footnote{For two records $v_1$ and $v_2$, it's negative correlated if $Pr(v_1=t)\geq Pr(v_1=t|v_2=t$).}
 if the inference result is within the previous knowledge of the adversary. So the
inference from correlation does not help.

With this assumption, we state the system privacy cost in Theorem \ref{theo-privacy-cost}.
\begin{theorem}
\label{theo-privacy-cost}
Given current differentially private system with query history , denoted by $\textbf{H}$ and privacy cost of all query , denoted by $\textbf{A}$,
the system privacy cost, denoted by $\bar{\alpha}$, can be derived from equation (\ref{fml-system-privacy}, \ref{fml-B}).
%Let $\textbf{B}$ be vector of used privacy budget of each cell, then
\begin{align}
\label{fml-system-privacy}
\bar{\alpha}=max(\textbf{B})
\\
\label{fml-B}
\textbf{B}=Sum_{row}(diag(\textbf{A}./\textbf{S})abs(\textbf{H}))
\end{align}
where $\textbf{B}$ be vector of used privacy budget of each cell,
function $diag()$ transforms a vector to a matrix with each of element in diagonal,
$Sum_{row}$ means the sum of rows.
\end{theorem}

\begin{proof}
First, we prove for each query $H_i$ in $\textbf{H}$, the privacy budget cost of each cell $x_j$ is $A_i/\textbf{S}_i*abs(H_i)$; then add up each cell and each row, we get the result.


%Let $\textbf{B}$ be the budget cost of all cells, $B_j$ be the budget cost of cell $x_j$.
For any query $Q$, the differentially private answer is returned as $\mathcal{A}_Q$.
Assume an adversary knows all the records of the data set except one record in cell $x_j$,
we define the local privacy cost for cell $x_j$ is $\alpha_j$
 if $\mathcal{A}_Q$ is $\alpha_j$-differentially private where
\begin{align}
\label{fml-budget-cost}
exp(\alpha_j)=\operatorname{sup}_{r\subseteq Range(Q)}\frac{Pr[\mathcal{A}_Q(D)=r | D=D_1]}{Pr[\mathcal{A}_Q(D)=r | D=D_2]}
\end{align}
where $D_1$ and $D_2$ are neighboring databases the same as definition \ref{def-DP}. Next we compute the local privacy cost of each cell for each query.


For each query $\textbf{H}_i$, the Laplace noise is $\tilde{N}(\textbf{A}_i/S_{H_i})$ according to equation (\ref{fml-lap-mec}).
By lemma \ref{lemma-GS} and equation (\ref{fml-SH}), it is $\tilde{N}(\textbf{A}_i/\textbf{S}_i)$. For the cell $x_j$,
assume an adversary knows all but one record in $x_j$, then the count numbers of other cells become constant in
this query. Thus this query becomes $\textbf{y}_i=\textbf{H}_{ij}\textbf{x}_j+\tilde{N}(\textbf{A}_i/\textbf{S}_i)+constant$.
The $S$ of this query is $H_{ij}$ and the noise of this query is $\tilde{N}(\textbf{A}_i/\textbf{S}_i)$. By Theorem \ref{theo-Lap-DP},
it guarantees $H_{ij} A_i/\textbf{S}_i$-differential privacy. Then the budget cost of $x_j$ is
$H_{ij} A_i/\textbf{S}_i$.


For example, in equation (\ref{fml-H}), $\textbf{H}_3=[0\ 0\ 0\ 0\ 4\ 2\ 0\ 0\ 0]$, $\textbf{x}_5=0$, $\textbf{x}_6=0$ by equation (\ref{eqn_x}), $\textbf{A}_3=0.05$ by equation (\ref{fml-A}).
According to equation (\ref{fml-y}), $\textbf{y}_3=\textbf{H}_3 \textbf{x}+\tilde{N}(\textbf{A}_3/4)=4\textbf{x}_5+2\textbf{x}_6+\tilde{N}(0.05/4)$.
For the cell $\textbf{x}_6$ with coefficient 2, assume an adversary knows all but one record in $\textbf{x}_6$, then the count numbers of other cells become constant in
this query.
So $\textbf{y}_3=4*0+2\textbf{x}_6+\tilde{N}(0.05/4)=2\textbf{x}_6+\tilde{N}(0.05/4)$.
The $S$ of this query is 2 and the noise of this query is $\tilde{N}(0.05/4)$. According to Theorem \ref{theo-Lap-DP},
it guarantees $0.025$-differential privacy. Then the local privacy cost of $\textbf{x}_6$ is $0.025$.
Similarly for $\textbf{x}_5$ with coefficient 4, $\textbf{y}_3=4\textbf{x}_5+\tilde{N}(0.05/4)$, so the local privacy cost of $\textbf{x}_5$ is $0.05$;
for $\textbf{x}_1$ with coefficient 0, $\textbf{y}_3=0*\textbf{x}_1+\tilde{N}(0.05/4)$, so the local privacy cost of $\textbf{x}_1$ is 0.

By theorem \ref{lemma-composition}, the local privacy cost composes linearly for all queries. Then the local privacy costs can add up by each query.

Because we assume cells are independent or negatively correlated in this paper,
 by Theorem \ref{lemma-parallel}, the privacy costs of all cells do not affect each other.
Therefore, we prove equation (\ref{fml-B}).

The highest privacy cost indicates the current system privacy cost, denoted by $\bar{\alpha}$.
So
we prove equation (\ref{fml-system-privacy}).
%
%The added noise is
%$\tilde{N}(A_i/max_{row}(|H_i|))$, by lemma \ref{theo-reverse-result} it guarantees $H_{ij}A_i/max_{row}(|H_i|)$-differential privacy.
%By theorem \ref{theo-equivalence-dp-ap}, the privacy budget cost for $x_j$ is $H_{ij}A_i/max_{row}(|H_i|)$. Finally, for all cells,
%the privacy budget costs for query $H_i$ is $|H_{i}|*A_i/max_{row}(|H_i|)$.
%
%To add all rows up, we just need to prove that sum of privacy budget costs for all queries is the budget cost for all queries.
%For each cell $x_j$, if there are 2 queries, $H_i$ and $H_{i+1}$, then we can assume the prior probability of adversary before $H_i$ is
%$Pr_{i-1}$, the posterior probability after $H_i$ is $Pr_{i}$; so the prior probability before query $H_{i+1}$ is $Pr_i$, and posterior
%probability after $H_{i+1}$ is $Pr_{i+1}$. Denote budget cost for $H_i$ and $H_{i+1}$ as $B_{i,i+1}$
%Recall definition \ref{def-budget-cost},
%\begin{align*}
%B_{i,i+1}=max (log(\frac{Pr_{i+1}(x_j| \mathcal{A}_{H_i,H_{i+1}})}{Pr_{i-1}(x_j)}))\\
%=max (log(\frac{Pr_{i+1}(x_j| \mathcal{A}_{H_i,H_{i+1}})}{Pr_{i}(x_j|\mathcal{A}_{H_i})} \frac{Pr_{i}(x_j|\mathcal{A}_{H_i})}{Pr_{i-1}(x_j)}) )\\
%=B_i+B_{i+1}
%\end{align*}
%
%Because $\textbf{H}$ is the all issued queries and $\textbf{A}$ is the used privacy budget for all these queries,
%$diag(\textbf{A})\textbf{H}$ is the exhausted privacy budget of each cell for all queries.
%By Theorem \ref{lemma-composition} and \ref{lemma-parallel}, the privacy budget in the each cell
%accumulates. Then $\textbf{B}=Sum_{row}(diag(\textbf{A})\textbf{H})$.
%Therefore, %the privacy budget costs for all queries linearly composes. Thus
%$\textbf{B}=Sum_{row}(diag(\textbf{A}./max_{row}(|\textbf{H}|))|\textbf{H}|)$.
\end{proof}

%\begin{theorem}[System privacy]
%\label{corollary-system-privacy}
%$\bar{\alpha}=max(\textbf{B})$
%\end{theorem}

In our example, we add $\textbf{H}_8=Q$ and $\textbf{A}_8=0.108$ to $\textbf{H}$ and $\textbf{A}$. Then by Theorem \ref{theo-privacy-cost}
\textbf{B} is in Equations (\ref{fml-result-B}).
system privacy $\bar{\alpha}$ is $0.408$ which is $max(\textbf{B})$.
Assuming the privacy budget for this system is 1, this would be
far less than the upper bound. Therefore, we return the differentially private answer from Laplace mechanism to user.
Finally, we update the parameters $\textbf{H}$, $\textbf{A}$ and $\textbf{y}$ for next coming query.
\begin{align}
\label{fml-result-B}
\small
\textbf{B}=
\left[
\begin{tabular}{ccccccccc}
         0  &  0.1 &        0    &     0   & 0.408 &   0.283   &      0  &  0.2 &   0.2
\end{tabular}
\right]
\end{align}


==> data/chap04.tex <==
\section{Simulation approach of probability function}
\label{sec-simulation-PDF}
%In this section, we discuss the PDF computation used in section \ref{cha3:sec-query-estimation}.

Detailed and sophisticated techniques about simulation approach can be found in \cite{book-statistical-inference,book-probability-models,book-Laplace}.
We introduce two methods to simulate the probability function in Section \ref{sec-simulate-PDF-1} and Section \ref{sec-combination-PDF-2}.
To achieve more accuracy, we compute the linear composition of probability function of Section \ref{sec-combination-PDF-2}.
%Section \ref{sec-simulate-PDF} discusses the simulation approach of probability function. Section
%\ref{sec-combination-PDF} discusses the linear computation of probability function. \ref{sec4-complexity} gives the computational complexity of the simulation approach.

































\subsection{Simulate probability function}
\label{sec-simulate-PDF-1}
We use a simulation approach to generate the probability function required in Algorithm \ref{alg-MMSE}.
Lemma \ref{lemma-principle} is proven in \cite{book-statistical-inference} by weak law of large number.
By this lemma, we derive
Theorem \ref{theo-PDF-n}, which is the main principle to derive simulated probability function.
Algorithm \ref{alg-simulation-PDF} describe the process of simulation. We use function $hist_X()$ as
$hist_X(t)=\sum_{i=1}^{m} b(X_i=t)/m$ where $b()$ is bool function.

\begin{lemma}
\label{lemma-principle}
Assume we know the probability function of $X$, Let $X_1,X_2,\\\cdots,X_{m_s}$ be i.i.d. random variables drawn from $PF_X$, then
\begin{align}
lim_{m_s\rightarrow \infty}Pr(|hist_X(t)-PF_{X}(t)|<\delta)=1
\end{align}
\end{lemma}

%
%\begin{lemma}
%\label{lemma-CDF}
%Assume $X_1,X_2,\cdots,X_{m_s}$ are i.i.d. random variables with Laplace distribution.
%if we use bool function to denote $X_i\leq t$ as $b(X_i\leq t)=1$, $b(X_i> t)=0$, then when $m_s$ is big enough, $\sum_{i=1}^{m_s}b(X_i\leq t)/m_s$ converges in probability to CDF of Laplace distribution,
%\begin{small}
%\begin{align}
%lim_{m_s\rightarrow \infty}Pr(|\sum_{i=1}^{m_s}b(X_i\leq t)/m_s-CDF_{X}(t,\alpha)|<\delta)=1
%\end{align}
%\end{small}
%where $CDF_{X}(t,\alpha)$ is the CDF of Laplace distribution with parameter $t$, $\delta$ is any arbitrarily small number.
%Proof in Appendix \ref{app-proof1}.
%\end{lemma}
%
%
%
%
%
%
%
%
%
%
%\begin{lemma}
%\label{lemma-PDF}
%Assume $X_1,X_2,\cdots,X_{m_s}$ are i.i.d. random variables with Laplace distribution,
%if we use bool function to present $X_i== t$ as $b(X_i= t)=1$, $b(X_i\neq t)=0$, then $\sum_{i=1}^{m_s}b(X_i= t)/m_s$ converges to PDF of Laplace distribution when $m_s$ is big enough.
%\begin{small}
%\begin{align}
%lim_{m_s\rightarrow \infty}Pr(|\sum_{i=1}^{m_s}b(X_i= t)/m_s-PDF_{X}(t,\alpha)|<\delta)=1
%\end{align}
%\end{small}
%\end{lemma}









\begin{theorem}
\label{theo-PDF-n}
Assume $[\textbf{X}_1,\textbf{X}_2,\cdots,\textbf{X}_{s}]$ is a
$m_s\times s$ matrix in which each element is a i.i.d. random variable with Laplace distribution, $\textbf{X}_j$ is the column of the matrix,
\begin{align}
Y_i=\sum_{j=1}^{s}\textbf{X}_{ij}
\end{align}
then $hist_Y(t)$ converges in probability to the probability function of sum of $s$ i.i.d. Laplace variables when $m_s$ is big enough,
\begin{align}
lim_{m_s\rightarrow \infty}Pr(|hist_Y(t)-f_s(t,\alpha)|<\delta)=1
\end{align}
where $f_s(t,\alpha)$is the probability function of sum of $s$ random Laplace variables.
\end{theorem}

%\begin{proof}
%According to Lemma \ref{lemma-PDF}, each $hist(\textbf{X}_j)$ converges to PDF of Laplace distribution,
%\begin{align}
%lim_{m_s\rightarrow \infty}hist(\textbf{X}_j)=PDF_{\textbf{X}}(b)
%\end{align}
%For each row in the matrix $[\textbf{X}_1,\textbf{X}_2,\cdots,\textbf{X}_{s}]$, $Y_i=\sum_{j=1}^{s}\textbf{X}_{ij}$ means $Y_i$ is derived from
%$s$ random Laplace variables. Similar to the proof of Lemma \ref{lemma-CDF} with Weak Law of Large Number\cite{book-Statistical-inference},
%we can prove $hist(\textbf{Y})$ converges in probability to PDF of sum of n i.i.d. random Laplace variables.
%\end{proof}




\begin{algorithm}[H]
\caption{Simulate discrete probability function of sum of s i.i.d Laplace noises $\sum_{j=1}^s\tilde{N}_j$}
\begin{algorithmic}
\label{alg-simulation-PDF}
\REQUIRE{$m_s$: sample size for a Laplace variable; $\alpha$: privacy budget}
\STATE
1. Draw a matrix $[\textbf{X}_1,\textbf{X}_2,\cdots,\textbf{X}_s]\in \mathbb{R}^{m_s\times s}$ of Laplace variables with probability function as equation (\ref{fml-Laplace-distribution}).\\
2. $\textbf{Y}=\sum_{j=1}^s \textbf{X}_{ij}$.\\
3. $\textbf{Y}=round(\textbf{Y})$.\\
4. $f_s(Y)={hist(\textbf{Y})}$.
\RETURN{simulated probability function $f_s(Y)$}
\end{algorithmic}
\end{algorithm}
Note that the probability function of Laplace distribution is symmetric. Therefore, for operator ``$-$'', we treat as ``$+$'', which will lead to the same result.


































\subsection{Linear computation of probability function}
\label{sec-combination-PDF-2}
%The more samples used, the higher the accuracy of the simulated probability function.
%Therefore,
%the computation cost for highly precise probability function would be expensive.
%Actually
%we can either simulate Laplace related probability function or compute discrete probability function of linear computation of n i.i.d. Laplace noises.
%Another reason for us to compute discrete probability function is that the posterior probability function will become different from Laplace distribution
%after computation with Equation (\ref{fml-PDF-theta-iteration}).

We define this problem as following:\\
$\textbf{N}=[\tilde{N}_1, \tilde{N}_2, \cdots, \tilde{N}_n]$ are $n$ noises and we know their probability functions(may not necessarily be Laplace distribution).
$T_i\tilde{\textbf{N}}$ is a linear computation of $\textbf{N}$ as equation (\ref{fml-TiN}).
we want to know the probability function of $T_i\tilde{\textbf{N}}$.
\begin{align}
\label{fml-TiN}
T_i\tilde{\textbf{N}}=t_1\tilde{N}_1+t_2\tilde{N}_2,\cdots,t_n\tilde{N}_n
\end{align}

To solve this problem, first we eliminate all coefficients by theorem \ref{theo-coefficients}.
Then As long as we solve operator ``$\pm$'', $T_i\tilde{\textbf{N}}$ can be solved by iteration.
Algorithm \ref{alg-combination-PDF} describes the process of linear computation of probability function.

\begin{theorem}
\label{theo-coefficients}
Probability function of $T_i\tilde{\textbf{N}}$ in equation (\ref{fml-TiN}) is the same as probability function of Z in equation (\ref{fml-TiN-Z}).
\begin{align}
\label{fml-TiN-Z}
Z=\tilde{N}_1'+\tilde{N}_2',\cdots,\tilde{N}_n'
\end{align}
where $\tilde{N}_j'=t_j\tilde{N}_j$ and $Pr_{\tilde{N}'}(\tilde{N}')={Pr_{\tilde{N}}(\tilde{N}'/t_j)}$.
\end{theorem}

\begin{algorithm}
\caption{Linear computation of probability function}
\begin{algorithmic}
\label{alg-combination-PDF}
\REQUIRE{$\tilde{\textbf{N}}$ with discrete probability function $Pr_{\tilde{\textbf{N}}}()$, $T_i$}
\STATE
1. $L_1(z) \leftarrow Pr_{\tilde{N}_1}(z/t_1)$ where $L$ is the result;\\
2. \FOR{each ${t_j \tilde{N}_j}$ in equation (\ref{fml-TiN}), $j\geq2$}
\STATE $Pr_{\tilde{N}'}(\tilde{N}')={Pr_{\tilde{N}}(\tilde{N}'/t_j)}$ by theorem \ref{theo-coefficients};
\FOR{each $k \in \mathbb{R}$}
\FOR{each $u,v \in \mathbb{R}$ where $u\pm v=k$}
    \STATE $L_j(k)\pm=L_{j-1}(u)Pr_{\tilde{N}_j'}(v)$;
\ENDFOR
\ENDFOR
\ENDFOR
\RETURN{probability function: $Pr_{T_i \tilde{\textbf{N}}}()=L(z)$}
\end{algorithmic}
\end{algorithm}

Note that in algorithm \ref{alg-combination-PDF} we will not compute all $k\in \mathbb{R}$ in practice, need to break the loop when $L_j(k)<negligible$ where $negligible$ is any predefined negligible small number.
We denote the range of $L_j(k)\geq negligible$ as the domain size of discrete probability function by $m_d$.

\subsection{Computational complexity}
%\label{sec4-complexity}
%\begin{theorem}
%\label{theo-complexity-1}
%If we consider $m_s$ as the sample size, $s$ as a constant, Algorithm \ref{alg-simulation-PDF} takes time $O(m_s)$.
%\end{theorem}
%\begin{proof}
%First, Drawing $sm_s$ random Laplace variables need $sm_s$ operations. Then step 2 takes time $sm_s$; step 3 takes time $m_s$; step 4 takes time
%$m_s$. So algorithm \ref{alg-simulation-PDF} takes time
%$O(m_s)$ where $m_s$ is the sample size for a Laplace variable.
%\end{proof}
\begin{theorem}
\label{theo-complexity-2}
If we consider $m_d$ as the domain size of each probability function,
$n$ as a constant, Algorithm \ref{alg-combination-PDF} takes time
$O(m_d^2)$.
\end{theorem}
\begin{proof}
For each operator $\pm$, for each domain value of the one probability function, it must traverse all the domain value of the other probability function. Therefore, each operator
$\pm$ takes time $m_d^2$. Then the algorithm takes time $O(m_d^2)$.
\end{proof}


==> data/chap05.tex <==
%\section{Security analysis of differential privacy}
%\label{sec-security-analysis}
%In this section, we first give the definition of adversarial privacy, then show that in practical case, the privacy leakage may not
%reach the theoretical bound $\alpha$ which is defined at the beginning. And the posterior PDF of any adversary can be quantitatively measured.
%
%\begin{definition}[Adversarial privacy]
%Assume an adversary has a prior PDF $Pr_0(t)$ w.r.t. a target victim in database $D$ where $t$ is the possible value of the sensitive attribute,
%a data access mechanism is
%$\alpha$-adversarial privacy if for all output $\tilde{\Theta}$, the equation holds:
%\begin{align}
%\label{fml-adversary-privacy}
%Pr_{post}(t|\tilde{\Theta})\leq e^\alpha Pr_0(t)
%\end{align}
%where $Pr_{post}(t|\tilde{\Theta})$ is the posterior PDF given $\tilde{\Theta}$.
%\end{definition}
%To measure the posterior PDF of the adversary, the main difficulty to adopt adversarial privacy is to choose the prior PDF,
%which is the power of the adversary. Provided with the PCNA(PTLM\cite{Rastogi-adversarial-privacy}), Laplace mechanism can be implemented
%for adversarial privacy. We are not going to discuss the PCNA class in this paper. Simply put, for independent records or negative correlation between records\footnote{For two records $v_1$ and $v_2$, it's negative correlated if $Pr(v_1=t)\geq Pr(v_1=t|v_2=t)$},
%the equivalence holds.
%
%\begin{theorem}
%Assume the attacker has a prior guess of a target victim with probability $Pr_0(t)$, after a set of queries $\textbf{Q}$ involving the target victim, ${\mathcal{A}}_{\textbf{Q}}(D)=\tilde{\Theta}$,
%\begin{align}
%\label{theo-Pr-post}
%Pr_{post}(t|\tilde{\Theta})\leq \frac{Pr_0(t)Pr(t|\tilde{\Theta})}{\int Pr_0(t)Pr(t|\tilde{\Theta})dt}
%\end{align}
%where $Pr_{post}(t|\tilde{\Theta})$is the posterior distribution.
%\end{theorem}
%\begin{proof}
%We show for the worst case, which assumes adversary knows all but the target victim records in the database, the operator ``='' holds in equation (\ref{theo-Pr-post}).
%Then for other types of adversaries, the operator ``<'' holds.
%
%Because the adversary knows all but the target victim, all the information in $\textbf{Q}$ can be eliminated except the target victim.
%Then the queries become the exclusive queries about target victim. Therefore, $Pr(\Theta=t|\tilde{\Theta})$ has the same shape with $Pr(victim |\tilde{\Theta})$.
%\end{proof}
%
%By the statistical inference introduced in section \ref{sec-online} and \ref{sec-simulation-PDF}, the bound of $Pr_{post}(t|\tilde{\Theta})$ can
%be derived. Further research on prior distribution $Pr_0(t)$ will lead to more precise result.








\section{}


==> data/chap06.tex <==

\section{Conclusion and future works}
\label{sec-conclusion} We have developed an efficient query
answering system with differential privacy. The system minimizes the
privacy cost for each query, maintains lower privacy budget usage,
can answer more queries and achieve a longer system life span. Our system is driven by utility, which is demanded by users.
Using the Bayesian inference technique,
we let users demand the credible interval and confidence level.
The returned answers include not only optimal credible interval but also optimal point estimation which achieves Minimal Mean Square Error.

This is the first paper that solve the statistical inference problem using Bayesian method.
The Bayesian inference method of this paper is an independent tool,
which  can also be used for other tasks, like disclosure risk analysis, parameter estimation
and other statistical inferences in future works.

The system can be improved by delicately designing the query history or using auxiliary queries.
Our greedy algorithm only optimize local budget usage because the computational complexity is too high.
Future works can research on how to
allocate least budget for a set of queries.
%Obtaining the bound of posterior distribution of adversarial privacy with our method, we believe it's
%useful for a series data publication with differential privacy.

\section{Acknowledgement}
This research was supported in part by NSF grant CNS-1117763, a
Cisco Research Award, and an Emory URC grant.

